On the detrimental effect of invariances in the likelihood for variational inference

Variational Bayesian posterior inference often requires simplifying approximations such as mean-field parametrisation to ensure tractability. However, prior work has associated the variational mean-field approximation for Bayesian neural networks with underfitting in the case of small datasets or large model sizes. In this work, we show that invariances in the likelihood function of over-parametrised models contribute to this phenomenon because these invariances complicate the structure of the posterior by introducing discrete and/or continuous modes which cannot be well approximated by Gaussian mean-field distributions. In particular, we show that the mean-field approximation has an additional gap in the evidence lower bound compared to a purpose-built posterior that takes into account the known invariances. Importantly, this invariance gap is not constant; it vanishes as the approximation reverts to the prior. We proceed by first considering translation invariances in a linear model with a single data point in detail. We show that, while the true posterior can be constructed from a mean-field parametrisation, this is achieved only if the objective function takes into account the invariance gap. Then, we transfer our analysis of the linear model to neural networks. Our analysis provides a framework for future work to explore solutions to the invariance problem.

==> sec/appendices/scaling.tex <==
\subsection{Scaling invariance}
Consider the model 
\begin{align}
\w &\sim p(\w) = \mathcal{N}(\w, \mu, \sigma^2), \\
\y &=  \prod_{k=1}^{K} \w_{k} + \epsilon,
\end{align}
where $\w$ is $K$-dimensional. This model is a product of Gaussian latent variables with a Gaussian likelihood with measurement noise $\epsilon$. 

This model has only 1 degree of freedom. Besides the permutation invariance (ignore here), we have a \emph{scaling invariance} that we could describe as a \emph{translation invariance in log-space}, similarly as above, on the $(K-1)$-dimensional hyperplane with normal vector $(1, 1, \dots, 1)$. 

This invariance can be described by the function 
\begin{align}
 f_{\rep}(\w) = \w \cdot  \mathbf{n}_{\rep} = \exp\left( \log \w + \log \mathbf{n}_{\rep} \right), \\
 f^{-1}_{\rep}(\bv) = \bv / \mathbf{n}_{\rep} = \exp\left( \log \bv - \log \mathbf{n}_{\rep} \right),
\end{align}
where $\log \mathbf{n}_{\rep}$ is any vector on the hyperplane that is perpendicular to its normal vector $(1, 1, \dots, 1)$. 

For example, with $K=2$ components, we have 1 degree of freedom, i.e.\ the line $\mathbf{n}_{\rep}= \rep \cdot (1, -1)$. 
\begin{align}
 f_{\rep}\begin{pmatrix} \w_1 \\ \w_2 \end{pmatrix} 
&= \begin{pmatrix} \w_1 \cdot \rep \\ \w_2 / \rep \end{pmatrix} 
= \begin{pmatrix} \bv_1 \\ \bv_2  \end{pmatrix} 
\\
f^{-1}_{\rep}\begin{pmatrix} \bv_1 \\ \bv_2 \end{pmatrix} 
&= \begin{pmatrix} \bv_1 / \rep \\ \bv_2 \cdot \rep \end{pmatrix} 
= \begin{pmatrix} \w_1 \\ \w_2  \end{pmatrix} 
\end{align}

This transformation is both \emph{bijective} (needs to be shown?) and \emph{volume-preserving}, since the determinant of the derivative is 
\begin{equation}
\left| \frac{d}{d \bv} f_{\rep}^{-1}(\bv) \right| = \frac{1}{\rep} \cdot \rep = 1.
\end{equation}





